BSharedRAG: Backbone Shared Retrieval-Augmented Generation for the E-commerce Domain

Retrieval Augmented Generation (RAG) system is important in domains such as e-commerce, which has many long-tail entities and frequently updated information. Most existing works adopt separate modules for retrieval and generation, which may be suboptimal since the retrieval task and the generation task cannot benefit from each other to improve performance. We propose a novel Backbone Shared RAG framework (BSharedRAG). It first uses a domain-specific corpus to continually pre-train a base model as a domain-specific backbone model and then trains two plug-and-play Low-Rank Adaptation (LoRA) modules based on the shared backbone to minimize retrieval and generation losses respectively. Experimental results indicate that our proposed BSharedRAG outperforms baseline models by 5% and 13% in Hit@3 upon two datasets in retrieval evaluation and by 23% in terms of BLEU-3 in generation evaluation. Our codes, models, and dataset are available at https://bsharedrag.github.io.

==> tables/ablation_gen.tex <==
\begin{table}[ht]
\centering
\small
\setlength\tabcolsep{2.6pt}
\begin{tabular}{lcccc}
\toprule
 \textbf{Model} & \textbf{BLEU} & \textbf{ROUGE-L} & \textbf{BertScore} & \textbf{Accuracy (\%)} \\
\hline
Ecom-RAG (ours) & 12.63 &12.85 &74.75 & 84.26 \\

% ~~~~ \textit{w/o} emb pretrain &  9.70 & 10.44 & 71.50& 80.86 \\
~~~~ \textit{w/o} chat pretrain &9.24 & 9.83 & 70.07 & 82.91 \\
~~~~ \textit{w/o} chat sft & 2.46 &3.24 & 62.58& 80.85\\
~~~~ \textit{w/o} chat pretrain \& sft & 2.32 & 2.49 & 62.56& 76.81\\

$\text{Ecom-RAG}_{\text{one\_lora}}$ & 2.35 & 2.58 & 62.37  & 68.34 \\

\bottomrule
\end{tabular}

\caption{}
\label{table:generation}
\end{table}

==> tables/ablation_retri.tex <==
\begin{table}[ht]
\centering
\small
% \setlength\tabcolsep{3.5pt}
\setlength\tabcolsep{3.6pt}
\begin{tabular}{lcccc}

\toprule
\multirow{2}*{\textbf{Model}} & \multicolumn{2}{c}{CPR-Ecom} &  \multicolumn{2}{c}{Ecom-PQA} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} 
~ & nDCG@3 & Hit@3  & nDCG@3 & Hit@3 \\ %指标统一，nDCG@3，Hit3 nDCG@5，
\midrule %字体new Times，Caption，横线移下来， w/o CL, w/o random negatives, w/o hard negatives, 实验支撑 bge finetune一下，继
% bge-base-zh & 56.91 & 7.39&73.90 &83.92 & 78.49& 50.74& & & \\
bge-large-zh& 51.25& 58.60 & 47.01 & 53.50 \\
~~~~\textit{w/}~ pre+hard-negative & 47.15 &58.10 & 45.38&51.20  \\
~~~~\textit{w/}~ hard-negative & 52.38 & 60.35 &48.46 &55.70  \\

Ecom-emb & \textbf{61.39} & \textbf{68.40}& \textbf{51.83}& \textbf{58.60}\\
~~~~\textit{w/o} pre & 56.74 & 63.80 & 49.02 &54.50\\
~~~~\textit{w/o} hard-negative  & 58.35 & 64.70 & 49.32 & 56.30 \\

\bottomrule
\end{tabular}

\caption{Ablation study on the pretraining and negative sampling methods}
\label{table:retrieve}
\end{table}

==> tables/ecom_retrie.tex <==
\begin{table}[!t]
\centering
\renewcommand{\arraystretch}{1.5}
\setlength\tabcolsep{3.6pt}
\small
\begin{tabular}{ lcccc } 

\hline
\textbf{Model}&\textbf{ nDCG@5}& \textbf{P@5}&\textbf{ R@5}& \textbf{F1@5}\\ \hline
m3e-large & 45.59 & 11.29& 10.14& 10.68\\ 

bge-large-zh & 49.86& 10.72& 10.83 & 11.56 \\ \hline

Ecom-emb (w/o pretrain) & 51.79 & 12.72 & 11.02 & 11.81 \\ 

Ecom-emb & \textbf{54.01} & \textbf{13.07} & \textbf{11.46} & \textbf{12.73} \\ 

\hline

\end{tabular}

\caption{ZDM-Ecom Retrieve Benchmark} 
\vspace{-2mm}
\label{table:ecom_retri} 
\end{table}


==> tables/generation.tex <==
\begin{table*}[ht]
\centering
\small
% \setlength\tabcolsep{3.5pt}
% \resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
 \textbf{Model} & \textbf{BLEU} & \textbf{ROUGE-L} & \textbf{BertScore} & \textbf{Accuracy (\%)} \\
\midrule 
GPT-3.5  & \textcolor{gray}{16.07} & \textcolor{gray}{12.76} & \textcolor{gray}{74.33} & \textcolor{gray}{86.77} \\
GPT-4\cite{openai2024gpt4} & \textcolor{gray}{19.76} & \textcolor{gray}{15.92} & \textcolor{gray}{77.98} & \textcolor{gray}{89.86}\\
EcomGPT\cite{li2024ecomgpt} & 6.91 & 8.12& 69.18 & 78.70 \\
Baichuan2-7b-base & 2.32 & 2.49 & 62.56& 76.81\\
Baichuan2-7b-base + continual training & 2.46 &3.24 & 62.58& 80.85\\
Baichuan2-7b-base + RAG instruction tuning &9.24 & 9.83 & 70.07 & 82.91 \\
Baichuan2-7b-chat\cite{yang2023baichuan} & 8.82 & 11.21 & 72.45 & 79.84 \\
Baichuan2-7b-chat + RAG instruction tuning &10.24 & 12.34& 72.12  & 82.33 \\

\cdashline{1-6}
\textbf{BShared-RAG (ours)}  & \textbf{12.63} &\textbf{12.85} &\textbf{74.75} & \textbf{84.26} \\
\text{FullyShared-RAG} & 2.35 & 2.58 & 62.37  & 68.34 \\
% ~~~~ \textit{w/o} emb pretrain &  9.70 & 10.44 & 71.50& 80.86 \\

\bottomrule
\end{tabular}

\caption{Evaluation of generation results based on our retriever on the WorthBuying-PQA test set.}
\label{table:generation}
\end{table*}

==> tables/halu.tex <==
\begin{table}[!t]
\setlength\tabcolsep{3.6pt}
\small
\centering
% \setlength\tabcolsep{3pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Model}  &  \textbf{Rej-rate} & \textbf{SRej-rate}& \textbf{QA-rel}&\textbf{ Faithfulness}
\\
\midrule
ChatGPT  \\
GPT-4   \\
EcomGPT      \\
Baichuan2-7B-chat  \\
\textbf{Ecom-chat} \\
~~~ w/o pre   \\
~~~ w/o IT & & & & \\
~~~ w/o Pre \& IT & & & & \\
\bottomrule
\end{tabular}
}
\caption{11}
\label{table:gen}
\end{table}

==> tex/01-intro.tex <==
\section{Introduction}
\textcolor{red}{why adapting RAG to a new domain is so important}
% Customers frequently seek answers to numerous product-related questions before making purchase decisions on e-commerce platforms, but the exponential growth of related content can lead to information overload and overwhelm consumers \cite{Roetzel2018Informationoverload}. Consequently, the Product Question Answering (PQA) task, aimed at providing precise and professional automated responses to product queries, has gained increasing scholarly attention in recent years \cite{deng-etal-2023-product}.
% directly integrating LLMs with external knowledge bases for domain-specific QA frequently poses challenges, as LLMs may have difficulty managing domain-specific knowledge \cite{zhang2024raft,siriwardhana-etal-2023-improving}. This difficulty highlights the need for further improvements. Domain-specific Continued Pre-Training (D-CPT) is an effective strategy to improve LLMs' domain comprehension \cite{ke2023continual,yıldız2024investigating_cp,que2024dcpt}. Therefore, combining Domain-Continued Pre-Training (D-CPT) with RAG may be a critical development in enhancing domain-specific QA capabilities.

Retrieval-Augmented Generation (RAG) effectively mitigates the issues of hallucinations and outdated knowledge in Large Language Models (LLMs) by incorporating external data sources \cite{zhu2024rag_survey,zhao2024ragsurvey3,gao2024ragsurvey2}. This integration renders RAG particularly advantageous for domain-specific question-answering (QA) tasks \cite{langchain,Liu_LlamaIndex_2022,zhang2024raft}. However, directly integrating LLMs with an external retrieval system may not suffice for domain-specific QA tasks in practical scenarios, as it faces challenges in adapting to domain-specific knowledge and contextual nuances \cite{zhang2024raft,siriwardhana-etal-2023-improving,zhang2023iag}. A crucial issue, therefore, is how to construct a domain-specific RAG system that is adaptively tailored to the needs of a specific domain, ensuring the integration is both effective and contextually appropriate.

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{figs/archcomp-v3.pdf}
\caption{\textbf{Three categories of possible RAG frameworks. The third one is what we proposed in this paper. } }
\label{fig:archcomp}
\end{figure*}


% \begin{figure}[!t]
% \centering
% \includegraphics[width=1.3\linewidth]{figs/example.pdf}
% \caption{\textbf{fig1} }
% \vspace{-5pt}
% \label{fig:1}
% \end{figure}

\textcolor{red}{todo: two important research questions}
In the construction of an effective domain-specific RAG system, there are mainly two challenges. The first challenge is the data problem. RAG requires a comprehensive knowledge database like Wikipedia for retrieval \cite{bolotova-baranova-etal-2023-wikihowqa,zhang2023iag,lin2023radit}. However, in domains such as e-commerce, high-quality expert knowledge from open sources is scarce. Existing datasets in e-commerce typically derive from user reviews on e-commerce platforms, which are generally brief and lack substantial information \cite{shen2023xpqa,JD,Taobao,amazonqa,deng-etal-2023-product}. A knowledge base lacking informative data may not effectively support the generation of LLMs \cite{zou2024poisonedrag,deng-etal-2023-product}.

% Previous research has explored retrieval-based models \cite{retrieveqa_1,retrieveqa_2,retrieveqa_3,bjerva-etal-2020-subjqa} and Seq2Seq generative-based models \cite{genqa_1, MAGEQA,shen-etal-2022-semipqa,genqa_2} using review-based PQA datasets, such as those from Amazon \cite{amazonqa} and JD \cite{JD}. Additionally, with the advancements in large language models (LLMs), numerous researchers \cite{li2024ecomgpt,peng2024ecellm,ma2023ecomgptct} have employed continual pre-training and instruction tuning methods to adapt LLMs for e-commerce tasks, including PQA. Moreover, e-commerce domain LLMs can be integrated with external embedding models to construct a Retrieval-Augmented Generation (RAG) framework to address PQA challenges more effectively \cite{Liu_LlamaIndex_2022,langchain}.

%Despite these efforts, the PQA task continues to face numerous challenges. Firstly, there is a substantial demand for high-quality open-source PQA datasets. Existing datasets \cite{icdm16-amazon,amazonqa,JD,Taobao,shen2023xpqa} from platforms like Amazon, JD, and Taobao consist of real user questions and review responses. These datasets often feature brief, non-expert responses, which can compromise accuracy, and many products lack corresponding QA pairs due to the long-tail effect in product distribution. Additionally, traditional RAG frameworks typically consist of an external BERT-style embedding model and domain-specific LLMs, which are trained independently. This separation means that embedding models cannot fully benefit from the continual pre-training stages of LLMs, making it difficult to adapt effectively to domain-specific scenarios such as PQA.

% Despite these efforts, adapting a general LLM to a specific domain continues to face numerous challenges. First, rather than relying an LLM, retrieval augmented generation is a must-have to meet a real user's demands for correct and high-quality answer; however, RAG frameworks involves multiple modules and datasets, which make it difficult to set up fair evaluations. Second, RAG frameworks typically consist of a BERT-style embedding model for retrieval and an LLM for generation, which have different architectures and separate training. As a result, the two embedding models cannot fully benefit from each other. Third, although there are some trials like \cite{GRIT} to use one LLM for both retrieval and generation, the full-parameter training and complex design to fit two different goals make it too heavy to be easily adapted to a new domain in real applications.

% Early works on Product Question Answering (PQA) also see this task as extracting relevant passage parts or retrieving relevant corpus from database or using a Seq2seq model to directly generate the answer.  
% In the field of E-commerce, product question answering (PQA) has become a crucial task \cite{deng-etal-2023-product}. Before deciding to purchase a product, consumers often extensively research product descriptions and reviews. However, the phenomenon of information overload \cite{Roetzel2018Informationoverload} can make this task overwhelming and exhausting due to the rapidly increasing volume of reviews and analytical articles. In this context, it is crucial to have a method that can automatically and accurately provide the information users seek. 
% Early works on Product Question Answering (PQA) can be categorized into three main approaches: treating PQA as a task of reading comprehension to extract relevant parts\cite{amazonqa,xu-etal-2019-bert,bjerva-etal-2020-subjqa}; considering it as a retrieval task to find relevant documents\cite{retrieveqa_1,retrieveqa_2,retrieveqa_3}; or using a Seq2seq model to directly generate responses \cite{genqa_1, MAGEQA,shen-etal-2022-semipqa,genqa_2}. However, due to the limitations of traditional models, the answers produced were often incomplete or too brief, which generally failed to satisfy users in real scenarios. Nowadays, Large Language Models (LLMs), such as  GPT-4 \cite{openai2024gpt4} and  Claude \cite{Claude}, have demonstrated excellent performance in various general natural language process tasks. There are also many works trying to apply LLMs to the E-commerce domain. 
% For example,  the works involving LLama-E\cite{shi2023llamae}, EcomGPT\cite{li2024ecomgpt}, and eCeLLM \cite{peng2024ecellm} have constructed instruction tuning datasets for the e-commerce domain and LLMs trained on these datasets have demonstrated a strong capability to follow instructions and excel in various e-commerce tasks, including PQA task. Meanwhile, Ecomgpt-CT \cite{ma2023ecomgptct} illustrates that domain-specific Continual training can further enhance the performance of LLMs across e-commerce tasks. Despite their effectiveness, these works struggle with timely knowledge updates and hallucination problems, which limit their application on the e-commerce platform. 
% Early works on the PQA can be categorized into three main approaches:  treating PQA as a task of reading comprehension to extract relevant parts \cite{amazonqa,xu-etal-2019-bert,bjerva-etal-2020-subjqa}; considering it as a retrieval task to find relevant documents\cite{retrieveqa_1,retrieveqa_2,retrieveqa_3}; or using a Seq2seq model to directly generate responses \cite{genqa_1, MAGEQA,shen-etal-2022-semipqa,genqa_2}. However, due to the limitations of traditional models, the answers produced were often too brief and unprofessional, which generally failed to satisfy users in real scenarios. Additionally, there is a significant shortage of high-quality datasets, particularly Chinese PQA datasets, which further complicates the development of effective solutions. With the emergence of Large Language Models (LLMs) \cite{openai2024gpt4, Claude}, some studies \cite{shi2023llamae,li2024ecomgpt,peng2024ecellm} have developed instruction-tuning datasets specifically for the e-commerce domain. These models are trained on these datasets and excel in various e-commerce tasks, including PQA. Despite their advancements, these LLMs still encounter issues with hallucinations and delays in knowledge updating, highlighting ongoing challenges in the field. \par
\textcolor{red}{todo: Our work for question one and question two}
% To address the first challenge, we.

% To address the second challenge, we.

% Previous research on Product Question Answering (PQA) faces several significant challenges, which we summarize as follows:
% (1) There is a notable absence of high-quality Chinese PQA datasets. Existing datasets predominantly feature reviews that are brief and primarily in English, underscoring the urgent need for comprehensive Chinese PQA datasets.
% (2) Traditional PQA methods, such as PAGE or other similar models, often generate responses that are overly concise and lack professional depth. This limitation indicates a need for a knowledge-rich model capable of addressing complex inquiries effectively.
% (3) E-commerce-specific Large Language Models (LLMs) encounter issues with hallucination and delays in updating knowledge, which can compromise the accuracy and relevance of the responses provided.

% Retrieval Augmented Generation (RAG) which introduces external information to LLMs can reduce problems such as hallucinations and untimely knowledge updating of LLMs\cite{zhu2024rag_survey,zhao2024ragsurvey3,gao2024ragsurvey2}. For PQA task , we can easily use off-the-shelf embedding models  and open-source LLMs with e-commerce  databases to significantly improve the performance. However, to the best of our knowledge, there is currently no research on RAG  specifically designed for the e-commerce domain. 

% Retrieval-Augmented Generation (RAG), which incorporates external information into Large Language Models (LLMs), appears to be an effective technology for mitigating issues such as hallucination, lack of professionalism, and delayed knowledge updates in LLMs \cite{zhu2024rag_survey,zhao2024ragsurvey3,gao2024ragsurvey2}. 
In this paper, we investigate how to adapt retrieval augmented generation to a domain effectively and efficiently. We introduce \textbf{WorthBuying-PQA}, a dataset comprising documents for pre-training and product question and answering (QA) in e-commerce domain and over 1.5 million QA pairs, to the public to facilitate research. %Unlike previous datasets of short reviews, WorthyBuying-PQA consists of long user generated content on product description and comparison.% We employ a hybrid method that combines real user queries and answers with LLM-generated QA pairs, ensuring each passage has two QA pairs. 
Second, we propose \textbf{SharedRAG}, a domain-adapted retrieval augmented generation framework. We first utilize domain-specific documents to continually pre-train a base LLM as a shared foundational model. Then we apply two Low-rank Adaptation (LoRA) modules to independently minimize the retrieval loss and generation loss. We conduct extensive experiments to compare our proposed SharedRAG framework with baselines, including full parameters fine-tuning the foundation model for retrieval and generation, and use one LoRA upon the foundation model to optimize retrieval and generation. Results indicate that our proposed method performs the best in both retrieval and generation evaluation. Detailed analysis shows that both continual pre-training and separated LoRA modules with shared foundation model contribute to the above improvements.%Interestingly, by avoiding using an %Our framework fully leverages the domain-specific continual pretraining by sharing the foundational model's parameters between the retriever and the generator. The two plug-and-play LoRA modules enable seamless switching between retrieval and generation, enhancing flexibility and performance.

% Given the above challenges,  we proposed \textbf{Ecom-RAG}, an \textbf{E-com}merce domain-specific \textbf{R}etrieval-\textbf{A}ugmented \textbf{G}eneration Framework. Retrieval-Augmented Generation (RAG), \cite{zhu2024rag_survey,zhao2024ragsurvey3,gao2024ragsurvey2} which incorporates external information into Large Language Models (LLMs), presents a promising solution to mitigate issues such as hallucinations, lack of professionalism, and delayed knowledge updates commonly associated with LLMs. Notably, we are the first to develop an E-commerce-specific RAG framework.
% First, we have constructed a high-quality Chinese Product Question Answering (PQA) dataset named Ecom-PQA. It is collected from a Chinese e-commerce website, SMZDM. To create this dataset, we designed a novel method that captures the complexity and diversity of consumer questions and answers. Our dataset includes 735,937 product descriptive articles, spanning 25 major product categories and 128 subcategories, thus offering a comprehensive resource for training and evaluating PQA systems in a real-world e-commerce environment. 
% Then, based on the Ecom-PQA dataset, we employ the E-commerce domain-specific continual pretraining method to train our framework's foundation model, \textbf{Ecom-base}. We build a novel architecture whose retrieval and generation parts are separately fine-tuned based on the foundation model Ecom-base. We use the E-commerce In-batch Negatives Contrastive Learning method and the E-commerce Retrieval-Augment Instruction Tuning method to train our retrieval model \textbf{Ecom-emb} and generation model \textbf{ Ecom-chat}.
% We conducted comprehensive experiments to validate the effectiveness of our Ecom-RAG framework. The results show that Ecom-emb outperforms existing embedding models on several e-commerce domain retrieval benchmarks. Overall, Ecom-RAG surpasses all baseline models on the PQA generation evaluation, including the GPT-4 \cite{openai2024gpt4} paired with the state-of-the-art retriever while utilizing only approximately 7B parameters. Thanks to our unique framework that does not incorporate additional embedding models, and with the help of the LoRA (low-rank adaptation) \cite{hu2021lora} method, our Ecom-RAG not only performs better than traditional architectures but also requires fewer parameters and less space.  \par
%We conduct extensive experiments to compare our proposed SharedRAG framework with baselines. Results indicate that our proposed method improves the best baselines in both retrieval and generation. %The retriever of SharedRAG achieves an average improvement of 7.85\% over the best BERT-style embedding model upon two e-commerce datasets for retrieval evaluation. The generator of SharedRAG significantly outperforms two open-sourced baselines in all metrics and achieves competitive performance with GPT3.5 in terms of ROUGE-L and BERTScore. 
%Detailed analysis shows that both continual pre-training and sharing foundation model contribute to the above improvements of retrieval and generation.%Interestingly, by avoiding using an external embedding model, Ecom-RAG has 4.3\% fewer parameters than the traditional RAG framework, while improving overall performance.

Our main contributions are as follows:
% \begin{enumerate}

$\bullet$ We construct a dataset called \textbf{WorthBuying-PQA} in e-commerce domain, which enables us to do continual pre-training and fine-tuning our RAG models. We will release the dataset to our community to facilitate further research.

$\bullet$ We propose the \textbf{SharedRAG} framework, which adapts an LLM to an e-commerce domain as a foundation model and builds two Low-rank Adaptation (LoRA) models based on the shared foundation model for both retrieval and generation.

$\bullet$ Experimental results demonstrate that SharedRAG, with affordable efficiency, outperforms traditional RAG methods in both retrieval and generation evaluation.
% \end{enumerate}


% Extensive experiments have demonstrated that our Ecom-RAG which has only about 7B parameters, has a better performance than several powerful baselines and needs a lower space cost.
% We first use the E-commerce domain-specific continual pretraining method to train an E-commerce-specific base model \textbf{Ecom-base}.  Ecom-base is enhanced using the Low-Rank Adaptation (LoRA) technique, where \textbf{Ecom-emb} is derived from the retrieval LoRA component via in-batch negative contrastive learning, and \textbf{Ecom-chat} is developed from the generation LoRA component through e-commerce Retrieval-Augmented Instruction Tuning. Ecom-RAG, combining a single foundational model with dual LoRA components for retrieval and generation, operates efficiently without the need for an additional Bert-style embedding model, ensuring streamlined functionality and coherence.\par
% In response to the scarcity of high-quality Chinese corpora for product question-answering tasks, We created the \textbf{ZDM-Ecom-Database }by standardizing and cleaning data from "Smzdm," a website known for its detailed product evaluations. We released it as an open-source retrieval database. This initiative aims to bolster research in e-commerce and natural language processing by improving access to comprehensive and informative datasets.
% We conduct extensive experiments to verify the effectiveness of our Ecom-RAG framework.  We conducted evaluations on the retrieval side and  generation side. On the retrieval side, we compare our Ecom-emb model with some common embedding models. Our Ecom-emb model both  excel baselines in the C-MTEB and ZDM-Ecom-Retrieve Benchmark.  On the generation side,  our Ecom-RAG framework which consists of Ecom-emb and Ecom-chat two models  outperforms all the same parameters baselines. Meanwhile, we test our space and time efficiency. Results show that our Ecom-RAG framework has a competitive space and time efficiency. 

==> tex/03-problem.tex <==
\section{Problem Formulation}
This paper aims to address the problem of question and answering in a specific domain, \eg, e-commerce, using a Retrieval-Augmented Generation (RAG) methodology. Our primary dataset for pretraining, referred to as $\mathcal{D}$, encompasses a corpus of e-commerce documents. The set is defined as follows:
\begin{equation*}
    \mathcal{D} = \{D_1,D_2,...,D_n\}
\end{equation*}
where $n$ denotes the number of documents within the corpus.

The RAG framework is composed of two main components: a retriever and a generator. When a query $\mathcal{q}$ is posed, the retriever identifies the top-k documents from $\mathcal{D}$ that are most relevant to the query. These documents are denoted as $\mathbf{d}_k$:
\begin{equation*}
\mathbf{d}_k = \text{Retriever}(q, \mathcal{D}, k) = \{d_i\}_{i=1}^k
\end{equation*}

For document retrieval, current methodologies often employ dense retrieval techniques using an embedding model $\phi$ to encode both documents and queries in a shared embedding space. The relevance of a document to a query is quantified based on the cosine similarity of their embedding. Tools like FAISS \cite{douze2024faiss} are commonly used to perform nearest neighbor searches in this embedded space and thus determine top-$k$ relevant documents:
\begin{equation*}
\mathbf{d}_k = \operatorname{arg\,max}_k \{ \text{sim}(\phi(d), \phi(q)) \mid d \in \mathcal{D} \}
\end{equation*}

Finally, the generator generates an answer $\mathcal{A}$ to the query $\mathcal{q}$ utilizing the retrieved documents $\mathbf{d}_k$ and its intrinsic knowledge via in-context learning methods \cite{ram2023incontext}:
\begin{equation*}
\mathcal{A} = \text{Generator}(q, \mathbf{d}_k)
\end{equation*}

It is crucial for RAG frameworks to enhance both performance of retriever and generator. A better retriever can capture more useful documents or a better generator can generate more accurate answers from the retrieved documents. In this paper, we aim to improve both by adapting a foundation model to the new domain and sharing the foundation model between retriever and generator.

==> tex/04-dataset.tex <==
\section{Data Preparation}

In this section, we provide details on data preparation. To effectively adapt a RAG framework to a new domain, we need to prepare six kinds of data in three phases. %First, we need documents in the new domain to complement to those general documents in continual pre-training phase to learn the domain's knowledge while keeping general one. Second, we need tuples of <query, positive document, negative document> to fine-tune the retriever of RAG framework. Again we need to mix the tuples in the new domain with those general to avoid losing general matching ability. Third, we need both general instructions, \ie, <question, answer>, and the domain-specific instructions, \ie, <question, document, answer> to fine-tune the generator of RAG. Thus the final model can maintain the ability to answer general questions while improving the ability to generate answer by referring the given document. 

%It needs To adapt a general RAG to a new domain.

%The Ecom-PQA dataset comprises 735,937 detailed product description passages and each passage contains two product-related QA-pairs. This section details the dataset's construction and compares it with prior works.
% 继续预训练：通用与专业比例5:1, 专业的
% 70万database for retrieval
% 检索微调：几万(百分比？)bge模型上开源的数据：query，pos doc, <neg doc1, neg doc2,...>, 几千电商数据：generated question, source doc, ranked docs - source doc, 10:1, general的能力（CMTEB榜还不错）没有降
% 面向RAG的指令微调（比通用多文章）：20万条开源的通用指令微调(Bellet通用指令)+5万条<generated question, source doc>最小化检索
\subsection{Data for Continual Training}
We need documents in the new domain to learn the domain's knowledge; however, if we use only these documents in continual pre-training, it is easy to forget general knowledge. Thus we prepare xxx documents in e-commerce domain and add five times documents in general domain for continual pre-training. The detailed data sources and quantities are provided in Table~\ref{fig:continualpretraining}. 

Among the e-commerce domain, we collect wiki pages of products and user generated articles that usually share some evaluation and experiences on products from a website called smzdm.com (a.k.a. What is Worthy Buying). Also we include user written notes after using some product from xiaohongshu.com (a popular website to share life guides). Moreover, we add articles on products and answers to a product related question from zhihu.com (a popular website to share profession opinions). Such documents contain rich knowledge on products. 

The process to create a high-quality, clean corpus involves:
\begin{enumerate}
\item \textbf{HTML cleanup and privacy protection.} We meticulously extracted content from the SMZDM website, ensuring the removal of HTML tags and any personally identifiable information to maintain user privacy.
\item \textbf{Deduplication and quality assessment.} We used a hashing method to eliminate duplicate entries. Additionally, engagement metrics such as likes, shares, and favorites were collected for each passage. These metrics were employed to derive a quality score for the articles, with only those scoring above a predetermined threshold included in the final dataset.
\end{enumerate}


The general documents are from Chinese wikipedia, web pages in common crawl, news, laws and patents. The ratios of difference sources are set empirically as shown in the Table~\ref{fig:continualpretraining}. Mixing them together can make it sure that our foundation model can perform well in both e-commerce domain and other general domains.

\begin{figure}[!t]
\centering
\includegraphics[width=1\linewidth]{figs/cp.png}
\caption{Data Recipe for Continual Pre-training}
\vspace{-1pt}
\label{fig:continualpretraining}
\end{figure}

% 70万database for retrieval
% 检索微调：几万(百分比？)bge模型上开源的数据：query，pos doc, <neg doc1, neg doc2,...>, 几千电商数据：generated question, source doc, ranked docs - source doc, 10:1, general的能力（CMTEB榜还不错）没有降

\subsection{Data for Fine-tuning Retrieval Model}
We need tuples of <query, positive document, negative document> to fine-tune the retriever of RAG framework. 
Again we mix the tuples in the new domain with those general to avoid losing general matching ability. The tuples from general domains are a subset of C-MTP (labeled) dataset~\cite{bge}. We also construct 50K tuples from e-commerce domains. In specific, we first sample 50K documents from the e-commerce domain. Then we leverage GPT-4 to generate a question for each document and thus the document is regarded as positive. Next, we propose using baseline models such as BGE \cite{bge} and M3E \cite{m3e}  to retrieve and rank documents from e-commerce database, which consists of 0.7 million documents in our experiments. Except for the positive document, those documents ranked at top 30 are regarded as hard negatives. The number of tuples in general domains is about ten times that in the e-commerce domain. As a result, our retrieval performance does not drop on some general retrieval benchmarks like CMTEB~\cite{bge} and the detail of the result is shown in the Appendix \ref{sec:appendix}.

% 面向RAG的指令微调（比通用多文章）：20万条开源的通用指令微调(Bellet通用指令)+5万条<generated question, source doc>最小化检索

\subsection{Data for Fine-tuning Generation Model}
We need both general instructions, \ie, <question, answer>, and the domain-specific instructions, \ie, <question, document, answer>, to fine-tune the generator of RAG. 
Our 200,000 general instructions are sampled from BELLET\cite{} while our domain-specific instructions are constructed by generating questions from sampled 50,000 e-commerce documents by leveraging an ask model. \textcolor{red}{give an example and describe the process.}
To mitigate the high costs of  API usage, we create a set of <question, document, answer> by using GPT-4 to generate the answer by taking the question and document in a prompt. Then we fine-tune an LLM to generate question. In parallel, we developed an 'answer' model capable of responding to both real and synthetic user queries based on the product context. This methodology allowed us to construct a dataset with high-quality question-answer pairs for each passage. 
Thus the final model can maintain the ability to answer general questions while improving the ability to generate answer by referring the given document. 

\subsection{Test Data of WorthBuying-PQA}
As indicated in Table \ref{tab:dataset}, previous Product Question Answering (PQA) datasets predominantly utilize English and are sourced primarily from Amazon. There is a noticeable scarcity of Chinese PQA datasets, with only the JD dataset \cite{wsdm19-answer-gen-gao} being open-sourced. Traditional datasets generally focus on product reviews or product information. However, these datasets often present limitations, such as a high proportion of unanswerable questions requiring extensive human annotation for answerability \cite{shen-etal-2023-xpqa, amazonqa}, and responses that are typically brief and challenging to verify for correctness.

To address these issues and enhance the dataset's professionalism and depth, our Ecom-PQA dataset updates the source of its content by utilizing a professional user review website as the primary data source. This shift ensures that the documents are not only longer but also richer in expert insights and technical details, making them more informative for research purposes. Our Ecom-PQA dataset employs a hybrid methodology to enhance the quality and depth of the data. This approach integrates authentic user inquiries with content generated by Large Language Models (LLMs), enriched with user perspectives. This innovative combination not only extends the average document length but also enriches the contextual quality of the information provided, making it highly relevant and comprehensive for each question. Consequently, this dataset significantly advances bilingual (Chinese and English) Product Question Answering (PQA) research by offering a uniquely detailed and user-focused resource.

%\subsection{Collection of Product-Related Passages}
%The dataset of product description passages was sourced from the SMZDM website, where users share product long reviews and evaluations. The process to create a high-quality, clean corpus involved:

%\begin{enumerate}
%\item \textbf{HTML cleanup and privacy protection.} We meticulously extracted content from the SMZDM website, ensuring the removal of HTML tags and any personally identifiable information to maintain user privacy.
%\item \textbf{Deduplication and quality assessment.} We used a hashing method to eliminate duplicate entries. Additionally, engagement metrics such as likes, shares, and favorites were collected for each passage. These metrics were employed to derive a quality score for the articles, with only those scoring above a predetermined threshold included in the final dataset.
%\end{enumerate}

%This streamlined method ensures the integrity and utility of the Ecom-PQA dataset, making it highly suitable for advanced research and applications in e-commerce product analysis.
\input{tables/dataset}
\begin{figure}[!t]
\centering
\includegraphics[width=1\linewidth]{figs/pqa_pie.png}
\caption{Distribution of Ecom-PQA categories and subcategories }
\vspace{-1pt}
\label{fig:2}
\end{figure}

%\subsection{User perspective question and answer generation}

%In real-world scenarios, many customer inquiries lack sufficient information to elicit appropriate responses, making them unanswerable and challenging for academic research. This situation frequently leads to a scarcity of high-quality user queries after filtering, which showcases a pronounced long-tail effect with inadequate user engagement for certain products. Additionally, responses from users on many platforms are unverified. Thus, it's still a great challenge for PQA dataset collection from many e-commerce platforms. To address the challenge, we utilize a hybrid methodology that blends authentic user-generated QA pairs with QA pairs generated by LLMs. 

%We initially collected authentic user questions from SMZDM website logs, cleaned the private information, and filtered out high-quality and answerable questions. By leveraging LLMs such as GPT-4, we can effectively simulate user queries that can ensure their answerability, diversity, and authenticity.  We use real scenarios QA-pair as in-context learning examples to leverage GPT-4 to ask questions and give answers based on product-related passages in the last section. 

%To mitigate the high costs of  API usage, we extracted a subset of the question-generating data from GPT-4 and trained a specialized 'ask' model. In parallel, we developed an 'answer' model capable of responding to both real and synthetic user queries based on the product context. This methodology allowed us to construct a dataset with high-quality question-answer pairs for each passage. The details of this part will be discussed in the appendix.

% To accurately reflect user inquiries and comprehend customer behavior in real e-commerce environments, we initially collected authentic user questions from SMZDM website logs. Due to the limited availability of such queries, we employed large language models (LLMs) to generate supplementary user queries derived from product-related content, ensuring that each passage was paired with a corresponding question and answer.

% We utilized GPT-4 for simulating user interactions through targeted prompt engineering, creating questions that align with the product descriptions. These artificially generated queries were integrated with real user questions to ensure comprehensive dataset coverage.

% To mitigate the high costs of continuous API usage, we extracted a subset of the question-generating data from GPT-4 and trained a specialized 'ask' model. In parallel, we developed an 'answer' model capable of responding to both real and synthetic user queries based on the product context. This methodology allowed us to construct a dataset with high-quality question-answer pairs for each passage.

 

%\subsection{Dataset Statistics and comparison with previous PQA datasets}
%As indicated in Table \ref{tab:dataset}, previous Product Question Answering (PQA) datasets predominantly utilize English and are sourced primarily from Amazon. There is a noticeable scarcity of Chinese PQA datasets, with only the JD dataset \cite{wsdm19-answer-gen-gao} being open-sourced. Traditional datasets generally focus on product reviews or product information. However, these datasets often present limitations, such as a high proportion of unanswerable questions requiring extensive human annotation for answerability \cite{shen-etal-2023-xpqa, amazonqa}, and responses that are typically brief and challenging to verify for correctness.

\begin{figure}[!t]
\centering
\includegraphics[width=1\linewidth]{figs/tradition.png}
\caption{Comparision with traditional RAG framework and our Ecom-RAG framework}
\vspace{-1pt}
\label{fig:tradition}
\end{figure}

%To address these issues and enhance the dataset's professionalism and depth, our Ecom-PQA dataset updates the source of its content by utilizing a professional user review website as the primary data source. This shift ensures that the documents are not only longer but also richer in expert insights and technical details, making them more informative for research purposes. Our Ecom-PQA dataset employs a hybrid methodology to enhance the quality and depth of the data. This approach integrates authentic user inquiries with content generated by Large Language Models (LLMs), enriched with user perspectives. This innovative combination not only extends the average document length but also enriches the contextual quality of the information provided, making it highly relevant and comprehensive for each question. Consequently, this dataset significantly advances bilingual (Chinese and English) Product Question Answering (PQA) research by offering a uniquely detailed and user-focused resource.

==> tex/05-method.tex <==
\section{Approach}


\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{figs/framework.pdf}
\caption{\textbf{Overview of the training stage and inference stage of Ecom-RAG Framework} }
%%% End Suggestion %%%
\vspace{-5pt}
\label{fig:framework}
\end{figure*}

\sun{In this section, we introduce our \textbf{Shared-RAG} framework for scenarios that require extensive domain knowledge, such as e-commerce. As shown in Fig.~\ref{fig:framework}, our framework is built on a shared foundation model for retrieval and generation. To train the foundation model to adapt to the specific domain, we first involve a domain-specific continual pertaining stage. Then we train the embedding and chat models based on the foundation model with two distinct LORA modules.}
\sun{maybe we can merge fig.4 and fig.5 to an overall framework.}


% \subsection{Overview Framework}
% Domain-specific continual pretraining has been an essential method to improve LLMs performance on specific domains\cite{xie2023efficient,ke2023continual,ma2023ecomgptct}. As depicted in Figure \ref{fig:tradition}, traditional RAG frameworks distinguish between the Retriever and Generator as separate entities, rendering the transfer of continual pretraining enhancements to the Retriever component challenging. The Ecom-RAG framework innovatively integrates the Retriever and Generator upon a unified base LLM, which undergoes continual pretraining specific to the e-commerce domain. This integration aims to optimize the utilization of domain-specific knowledge throughout the continual pretraining process. 

% Within the Ecom-RAG, we first employ the domain-specific continual pretraining method to train an e-commerce domain professional model called \textbf{Ecom-base} as our foundation model. Then, we use the low-rank adaption method (LoRA) \cite{hu2021lora} to train our embedding model and generation model based on our Ecom-base. Our embedding model, named \textbf{Ecom-emb}, uses a novel method called e-commerce In-batch Negatives Contrastive Learning inspired by DPR\cite{dpr}, but with the backbone model initialized with Ecom-base. Our generation model, named \textbf{Ecom-chat}, has been specifically developed through e-commerce Retrieval-Augmented Instruction Tuning. This technique is designed to enhance the model's proficiency in e-commerce contexts and its ability to extract relevant information effectively. 

% Fig \ref{fig:tradition} clearly shows the training stage and inference stage of our Ecom-RAG framework.  The training stage consists of three phases: e-commerce domain-specific continual pre-training, e-commerce In-batch Negatives Contrastive Learning, and e-commerce Retrieval Augmented Instruction Tuning. During the inference stage, the Ecom-emb—comprising the Ecom-base and retrieval LoRa—serves as the primary embedding model. This model proficiently encodes queries into embedding vectors. Subsequently, these vectors facilitate a targeted search within the Ecom-PQA corpus. The retrieved results are then amalgamated with the initial query, forming a composite input for the Ecom-chat, our generative model. This model adeptly synthesizes the composite input to generate precise and contextually relevant answers. This streamlined process underscores our framework’s capability to integrate and apply specialized e-commerce knowledge effectively during real-time inquiries. 



\subsection{\sun{Domain-specific Continual Pretraining}
% e-commerce domain-specific continual pertaining
}
\sun{To adapt a general foundation model to a specific domain, we employ a domain-specific continual pretraining approach to train the foundational model. In our case of e-commerce, we build a high-quality e-commerce corpus from the Ecom-PQA dataset. To mitigate the catastrophic knowledge collapse of the foundation model, following~\cite{xie2023efficient,ke2023continual,que2024dcpt}, we also integrate some general data into the training corpus.}
% During this phase, we employ a domain-specific continual pretraining approach to train our foundational e-commerce model, Ecom-base.  The continual pre-training connects the stages of general pertaining and supervised fine-tuning. Firstly, we integrate a high-quality e-commerce corpus from Ecom-PQA with general data to create a domain-specific dataset for continual pertaining.
Then, we implement a comprehensive pipeline for data reformulation, filtering, and deduplication to ensure high-quality and clean data. \sun{We include more details in the Appendix Sec.~\ref{}}
% Like EcomGPT-CT \cite{ma2023ecomgptct}, we gather e-commerce domain corpora from diverse sources, mixing this data with general domain corpora.  

The domain-specific continual pretraining objective is the next token prediction task, the same as the general \sun{language model} pretraining stage: 
\begin{equation*}
    max_{\theta}~\sum_{i=1}^N~log~P(y_i|y_{<i};\theta)
\end{equation*}
where $\theta$ is the parameter of \sun{the foundation} LLMs
% (Here is Baichuan2-7B-Base \cite{yang2023baichuan}) 
and $y$ is a training text sequence.
% In this approach, we integrate a high-quality e-commerce corpus from Ecom-PQA with general data to create a domain-specific dataset for continual pretraining. Subsequent experiments demonstrate that this method indeed enhances model performance.

\sun{This paragraph can be placed in the implementation details.}
% We utilize the Hugging Face framework \cite{wolf2020huggingfaces} and adopt data parallelism via DeepSpeed ZeRO Stage 2 \cite{rajbhandari2020zero}. Training is conducted with bfloat16 precision and a learning rate of 1e-5 on 4 Nvidia H100s for approximately 190 hours, utilizing a pretraining corpus of about 100GB with activation checkpointing enabled.  Further details regarding our continual pretraining approach are provided in Appendix .

% \subsection{e-commerce In-batch Negatives Contrastive Learning}
\subsection{\sun{Shared Foundation Model for Retrieval and Generation}}

\sun{RAG is an important technique for incorporating external knowledge into LLMs.
Previous works leverage a separate embedding model for retrieval and an LLM for answering.
This paradigm has two main shortcomings: firstly, both the embedding model and the answer model require domain-specific adaptation through continual pre-training to better fit new domains; secondly, traditional embedding models rely on smaller-scale models such as BERT, which may result in suboptimal retrieval performance. In this paper, we propose a unified approach where both the embedding and the answer model are based on the same shared foundational model, \ie, a Large Language Model (LLM). The advantage of this approach is that we can focus on domain-specific pre-training of the foundational model only, and then employ lightweight modules such as LoAR for retrieval and generation tasks. This also allows the retrieval model to leverage the capabilities of the LLM. Compared to separately adapting the retrieval and generation models to the domain, our approach also reduces training costs and simplifies the training process. 
}

\paragraph{\sun{Training Embedding Model with Hard Negative Mining.}}
\sun{
We fine-tune a domain-specific embedding model to enhance performance based on a frozen base LLM with trainable LoRA modules. Our embedding model adopts a GPT-like architecture, we adhere to the RepLLaMA paradigm \cite{ma2023repllama} to derive sentence embeddings from the End of Sentence (EOS) token.
}

Following the approach of the bi-encoder dense retriever DPR \cite{dpr}, we employ in-batch contrastive learning to fine-tune Ecom-base. We utilize the InfoNCE Loss function:

\begin{equation*}
\mathcal{L} = -\log \frac{e^{sim(q,D^+)}}{e^{sim(q,D^+)}+\sum_{D_i^- \in {D^-}}e^{sim(q,D_i^-)}}
\end{equation*}

Here, $D^+$ represents the relevant document, and ${D^-}$ denotes a set of irrelevant documents to the query. We employ the in-batch negatives method, where one positive document and several negative documents are included in one sample.
We also propose a strategy for identifying hard negatives during contrastive learning. Specifically, we utilize a baseline embedding model to retrieve a preliminary set of potential negatives, then the high-ranking yet erroneously matched documents—termed "hard negatives." These documents provide the crucial examples needed to refine the model’s discrimination capabilities.

% Embedding models play a crucial role in encoding text into semantic embedding representations. Leveraging Ecom-base as the foundation, we fine-tune an e-commerce domain-specialized embedding model to enhance performance in product question-answering tasks. 

% A key challenge in embedding models lies in extracting embeddings from the model. Previous approaches, such as those based on Bert-style embedding models, typically utilize the representation of the [CLS] token as the dense representation of the input text. However, which adopts a GPT-like architecture, we adhere to the RepLLaMA paradigm \cite{ma2023repllama}, pooling the embedding using the special token "</s>". The embeddings of queries and documents are computed as follows: 
% \begin{equation*}
%     E = Ecom\_emb(``t_1t_2...t_k</s>")[-1]
%     \nonumber
% \end{equation*}
% % Recent research \cite{jiang2023scaling} explores the impact of well-designed prompts on enhancing the embedding representation of Language Models (LLMs). In our approach, we employ the default prompt from Repllama uniformly for instruction prompts. Specifically, for queries, we prepend "query:" to the text, and for documents, we prepend "document:" to the text.  Further investigation into the effects of instruction prompts will be conducted in section 6, allowing for a comprehensive understanding of their influence on model performance.
% Following the approach of the bi-encoder dense retriever DPR \cite{dpr}, we employ in-batch contrastive learning to fine-tune Ecom-base. We utilize the InfoNCE Loss function:

% \begin{equation*}
% \mathcal{L} = -\log \frac{e^{sim(q,D^+)}}{e^{sim(q,D^+)}+\sum_{D_i^- \in {D^-}}e^{sim(q,D_i^-)}}
% \end{equation*}

% Here, $D^+$ represents the relevant document, and ${D^-}$ denotes a set of irrelevant documents to the query. We employ the in-batch negatives method, where one positive document and several negative documents are included in one sample.

% To address the challenge of identifying hard negatives in the e-commerce domain, we devised a domain-specific technique for mining these difficult examples. Initially, a baseline embedding model retrieves a preliminary set of potential negatives. Subsequently, through manual annotation, we identify high-ranking yet erroneously matched documents—termed "hard negatives." These documents are ranked high by the retrieval model but are incorrect, thereby providing the crucial examples needed to refine the model’s discrimination capabilities.

% This targeted approach enhances the model's ability to discern nuanced differences between similar e-commerce items, improving its overall performance in product-related queries. The training of Ecom-emb incorporates these hard negatives, significantly boosting the model's effectiveness in practical scenarios. This process is comprehensively detailed in the Appendix, describing the adaptations made to the standard in-batch negatives method and the subsequent training on Nvidia H100 80GB GPUs.

\paragraph{\sun{Training Generation Model with Retrieval Augmented Instruction Tuning.}}

\sun{
We introduce a domain-specific retrieval-augmented instruction tuning to train the generator. To improve the generator's capability of effectively utilizing retrieved information, we augment the instruction-response pairs by incorporating articles retrieved by the retriever, forming instruction-article-response triples. Similar to the embedding model, we employ LoRA module to fine-tune only a subset of additional parameters on the top of foundational LLM.}

% \subsection{e-commerce Retrieval Augmented Instruction Tuning}
% In the training of Ecom-chat, we introduce a method termed e-commerce Retrieval-Augmented Instruction Tuning. Initially, inspired by prior works such as EcomGPT \cite{li2024ecomgpt} and Ecellm \cite{peng2024ecellm}, we construct a specialized instruction tuning dataset tailored to the e-commerce domain, leveraging the capabilities of the GPT-4 API. This dataset is meticulously designed to enhance the language model's proficiency in understanding and generating e-commerce-related content.

% Moreover, to strengthen the language model's capacity to effectively utilize retrieved information, we augment the dataset by incorporating contextual cues extracted from e-commerce articles. This augmentation strategy aims to enrich the training data with real-world e-commerce contexts, enabling the model to better comprehend and respond to diverse scenarios encountered in e-commerce interactions. Our approach combines both domain-specific instruction tuning data and Retrieval-Augmented instruction tuning, resulting in a comprehensive e-commerce Retrieval-Augmented Instruction Tuning dataset. This dataset serves as the foundation for training Ecom-chat, facilitating the development of a specialized conversational model tailored to the intricacies of the e-commerce domain.

% Same as Ecom-emb, we employ the LoRA training method, focusing on fine-tuning only a subset of additional parameters. All training procedures are conducted on four Nvidia H100 80GB GPUs, with a total training time of 1.5 hours. Further details regarding the training of Ecom-chat are provided in the Appendix.
